Asset Bundling for Wind Power Forecasting

The growing penetration of intermittent, renewable generation in US power grids, especially wind and solar generation, results in increased operational uncertainty. In that context, accurate forecasts are critical, especially for wind generation, which exhibits large variability and is historically harder to predict. To overcome this challenge, this work proposes a novel Bundle-Predict-Reconcile (BPR) framework that integrates asset bundling, machine learning, and forecast reconciliation techniques. The BPR framework first learns an intermediate hierarchy level (the bundles), then predicts wind power at the asset, bundle, and fleet level, and finally reconciles all forecasts to ensure consistency. This approach effectively introduces an auxiliary learning task (predicting the bundle-level time series) to help the main learning tasks. The paper also introduces new asset-bundling criteria that capture the spatio-temporal dynamics of wind power time series. Extensive numerical experiments are conducted on an industry-size dataset of 283 wind farms in the MISO footprint. The experiments consider short-term and day-ahead forecasts, and evaluates a large variety of forecasting models that include weather predictions as covariates. The results demonstrate the benefits of BPR, which consistently and significantly improves forecast accuracy over baselines, especially at the fleet level.

==> tex/1.1_hierarchical_reconciliation.tex <==
\section{Hierarchical Forecast Reconciliation}
\label{sec:reconcilation}





By bundling the generators together, it naturally created a hierarchical structure for the forecasts. One can see this forecast hierarchy in three levels, the first is total level, which is a forecast on total wind power, the second level is the bundle-level, which is aggregated via proposed bundling methods. The bottom level is the generator-level. Bundling wind farms and forecasting at the bundle-level may lead to a loss of precision at the generator level due to aggregation. Nevertheless, predicting wind power for each generator is less accurate after aggregated. The objective of hierarchical reconciliation is to leverage forecasts at different levels to provide the most accurate and coherent forecasts for all levels in the hierarchical structure.

For a fixed time point $t$, the hierarchical measures of generator level generation $x_{1,t},...,x_{N,t}$, bundle level $z_{1,t},..., z,...,z_{N,t}$, and total level $y_{t} = \sum_{i = 1}^{N} x_{i,t}$ can be decomposed into a summing matrix $\mathcal{S}$ of size $(N + K + 1) \times N$ and generator-level measures,

\begin{equation}
\mathbf{h}_t = 
\begin{bmatrix}
 y_{t}\\
z_{1,t} \\ 
\vdots \\
z_{K,t} \\
x_{1,t} \\ 
\vdots \\
x_{N,t}  
\end{bmatrix} 
= 
\begin{bmatrix}
    1 & 1 & \cdots & 1 \\
    \lambda_{1,1} & \lambda_{1,2} & \cdots & \lambda_{1,N} \\
    & & \ddots& \\
    \lambda_{K,1} & \lambda_{K,2} & \cdots & \lambda_{K,N} \\
    1 & 0 & \cdots & 0 \\
    0 & \ddots & \cdots & 0 \\
    0 & 0 & \cdots & 1 
\end{bmatrix} 
\begin{bmatrix}
    x_{1,t} \\ 
    \vdots \\
    x_{N,t}  
\end{bmatrix} = \mathcal{S} \mathbf{x}_t.
\label{eq:hierarchical decomposition}
\end{equation}
The first row of the summing matrix $\mathcal{S}$ indicates that the total wind power is the sum of all power generated by the $N$ generators. Rows two to $K+1$ indicate that each bundle should sum the individual generations within the bundle. The last $N$ rows are an identity matrix $I_{N}$, indicating that generator-level measures are exactly $\mathbf{x}_t$. This transformation enables the transition from generator-level measures to coherent hierarchical measures. 

In the forecasting context, predictions are obtained for all levels in the hierarchical structure, denoted as
$\mathbf{\hat{h}}_{t} = \begin{bmatrix}
\hat{y}_{t}\\
\mathbf{\hat{z}}_{t} \\ 
\mathbf{\hat{x}}_{t} \\ 
\end{bmatrix}
$, where each forecast in the matrix can originate from different forecasting models and may not necessarily be coherent across levels. Linear hierarchically coherent forecasts are represented as:
\begin{equation}
     \mathbf{\Tilde{h}}_{\tau}  = \mathcal{S} \mathcal{G}_{\tau} \mathbf{\hat{h}}_{\tau},
\end{equation}
where $\mathcal{G}_{\tau}$ is a matrix that reconciles the generator-level forecast at time dimension $\tau$, and $\mathcal{S}$ maps the base-level forecast to a hierarchical forecast. Therefore, the problem becomes to find the optimal $G_{\tau}$.  One of the property that is desired is is the hierarchical forecast is unbiased given the generator-level forecasts are unbiased. This so-called unbiased preserving constraint on $G_\tau$ is introduced in \cite{hyndman2011optimal} as $\mathcal{S}\mathcal{G}_{\tau}\mathcal{S} = \mathcal{S}$. 

There are different approaches to implement $\mathcal{G}$. In this paper, Minimum Trace (MinT) optimal reconciliation approach approach proposed by Wickramasuriya et al. has been implemented \cite{minT2019}, which show that the optimal $G$ that minimizes the error variances of the coherent forecasts and satisfies the unbiased preserving constraint is given by $\mathcal{G} = (\mathcal{S}' \mathbf{W}_\mathcal{T}^{-1}\mathcal{S})^{-1}\mathcal{S}'\mathbf{W}_\mathcal{T}^{-1}$, where $\mathbf{W}_\mathcal{T}$ is the variance-covariance matrix of the $T$-step forecast error. There are many ways to estimate $\mathbf{W}_\mathcal{T}$. We use the weighted least square applying variance scaling ($\text{WLS}_v$) approach as described in \cite{minT2019} with slight modification. $\mathbf{W}_{\tau} = k_{\tau} \text{diag} (\hat{\mathbf{W}_{\tau}})$, where $k_{\tau} > 0$, 
\begin{equation}
    \mathbf{\hat{W}}_{\tau} = \frac{1}{M} \sum_{t \in \mathcal{M}} \mathbf{e}_{t,\tau}\mathbf{e}_{t,\tau}'
\end{equation},
where $\mathbf{e}_{t,\tau}$ is an $N + k + 1$ dimensional vector of in-sample error of the model at time dimension $\tau$. 

In our experiment, the ols approach, MinT(sample), OLS, and $\text{wls}_{s}$ are also tested. However, the $\text{wls}_v$ method has the overall best performance. 
\hz{mention somewhere that mint-cov and ols are also used, but performance are not as good. }
